Stochastic approximation approaches for CVaR-based variational inequalities

This paper considers variational inequalities (VI) defined by the conditional value-at-risk (CVaR) of uncertain functions and provides three stochastic approximation schemes to solve them. All methods use an empirical estimate of the CVaR at each iteration. The first algorithm constrains the iterates to the feasible set using projection. To overcome the computational burden of projections, the second one handles inequality and equality constraints defining the feasible set differently. Particularly, projection onto to the affine subspace defined by the equality constraints is achieved by matrix multiplication and inequalities are handled by using penalty functions. Finally, the third algorithm discards projections altogether by introducing multiplier updates. We establish asymptotic convergence of all our schemes to any arbitrary neighborhood of the solution of the VI. A simulation example concerning a network routing game illustrates our theoretical findings.

==> subspace.tex <==

	



\clearpage

	In this section we take a more detailed look at the case where $\HH$ is of the form \eqref{explicit contrained set 2}. Specifically we look at an alternative way to handle the equality constraints $r^j(h) = 0$ for all $j \in [l]$. Since the functions $r^j(\cdot)$ are affine, we can summarize all equality constraints in the compact notation
	\begin{equation*}
		Ah = b,
	\end{equation*}
	where $A \in \real^{l \times n}$ and $b \in \real^l$ are chosen appropriately. Since the solution $h^*$ of $\VI(\HH,F)$ is in $\HH$ we have $Ah^* = b$. Naturally, any algorithm for finding $h^*$ should therefore converge to the set $\setdef{h \in \real^n}{Ah = b}$. However, if we can make an initial guess $h_0$ such that $Ah_0 = b$ it is often preferable that the iterates $h_i$ \emph{stay} in this set, preferably without the need for calculating projections. In other words, if $Ah_0 = b$ and we have $h^{k+1} = h^k - \gamma^k G(h^k)$, a nice property to have would be
	\begin{equation*}
		A G(h^k) = 0.
	\end{equation*}
	This would guarantuee that $A h^k = b$ for all $k$. Letting $-\tilde{G}(h^k)$ be the direction in which an algorithm would move in the $k$-th iteration, we can let $-G(h^k)$ be the projection of $-\tilde{G}(h^k)$  onto the \emph{subspace} $\setdef{f \in \real^n}{Af = 0}$. Projection onto this subspace can be achieved with a linear map $L$ which can be calculated at the start of the algorithm as follows:  Let $\{a_1,\cdots,a_t\}$ be the row vectors of $A$, and let $\{u_1,\cdots,u_n\}$ be an orthonormal basis for $\mathbb{R}^n$ such that the first $M \in \naturalnumbers$ vectors $\{u_1,\cdots,u_{M}\}$ form a basis for $\text{span}(a_1,\cdots,a_l)$. Then we have [REFERENCE]
	\begin{equation*}
		\Pi_{\setdef{g \in \real^n}{Ag = 0}}(G) = (I - \sum_{i = 1}^{M} u_i u_i^T)G.
	\end{equation*}
	We see that projection onto the subspace is achieved via the linear map $L$ defined by
	\begin{equation} \label{eq:subspace-projection-matrix}
		L := (I - \sum_{i = 1}^{M} u_i u_i^T).
	\end{equation}
	The following illustrates how we can apply this concept to our previously designed algorithms.
	%
	%
	\todoa{What bothers me in the following algorithm is the fact that we are still doing the projection onto the set $\HH$ of a point. Don't we want to get rid of that nasty projection now that we have already dealt with the inequalities?}
	%
	\begin{proposition}
		Let the assumptions of Proposition \ref{penalty theorem} hold, where $\HH$ is of the form \eqref{explicit contrained set 2} and \eqref{penalty algorithm} is replaced with
		\begin{equation*}
			h^{k+1} = h^k -\gamma^k L \Big(F(h^k) + c\big(h^k - \Pi_{\HH}(h^k)\big) + \widehat{\beta}^{N_k}\Big).
		\end{equation*}
		Here $L$ is as defined in \eqref{eq:subspace-projection-matrix} and we assume that $Ah^0 = v$. Then, for any $\epsilon > 0$ there exist $c_\epsilon > 0$ and $N_\epsilon \in \naturalnumbers$ such that when $c_P > c_\epsilon$ and $N_k \geq N_\epsilon$ for all $k$ then, with probability one,
		\begin{equation*}
			\lim_{k \rightarrow \infty}\norm{h^k - h^*} \leq \epsilon.
		\end{equation*}
	\end{proposition}
	\begin{proof}
		First we note that $A h^k = b$ for all $k$. To see this, let $a_i$ denote a row of $A$. It follows that there exist $c_j \in \real$ such that $a_i = \sum_{j = 1}^r c_j u_j$. This gives us
		\begin{align*}
			a_i^\top L &= a_i^\top - \sum_{j = 1}^{M} c_j u_j^\top \sum_{i = 1}^{M} u_i u_i^\top 	\\
			&= a_i^\top - \sum_{j = 1}^{M} c_j u_j	\\
			&=  a_i^\top -  a_i^\top = 0.
		\end{align*} 
		Therefore we have $A L = 0$. It follows that $A h^{k+1} = A h^k$ and since $A h^0 = b$ we have $A h^k = b$ for all $k$.
		Let
		\begin{equation*}
			G(\bar{h}(t)) :=  F\big(\bar{h}(t)\big)  -  c\Big(\bar{h}(t)  -  \Pi_{\HH}\big(\bar{h}(t) \big) \Big) \! - \! \bar{b}(t).
		\end{equation*} Analoguous to the proof of Proposition \ref{projected theorem}, it can be established that $\{h^k \}$ converges, in the sense of \eqref{eq:convergence to trajectory}, to a trajectory satisfying
		%\begin{subequations}\label{eq:ODE-h-lm-2}
		\begin{equation} \label{eq:subspace-ODE}
			\dot{\bar{h}}(t) = -L G\big(\bar{h}(t)\big)
			%\frac{d}{d t} \bar{h}(t)  =  -L\bigg(F\big(\bar{h}(t)\big) \! - \! c\Big(\bar{h}(t)  \!- \! \Pi_{\HH}\big(\bar{h}(t) \big) \Big) \! - \! \bar{b}(t)\bigg)
			%   \dot{\bar{h}}(t) &= -F\big(\bar{h}(t)\big) - Dq\big(\bar{h}(t)\big)^\top \bar{\lambda}(t) - Dl\big(\bar{h}(t)\big)^\top \bar{\mu}(t) - \bar{b}(t), \label{ODE h part} \\ 
			%\dot{\bar{h}}(t) &= -L \Big( H\big(\bar{h}(t), \bar{\lambda}(t), \bar{\mu}(t)\big)  - \bar{b}(t) \Big)    \\
			%\dot{\bar{\lambda}}(t) &= \Big[q\big(\bar{h}(t)\big)\Big]_{\bar{\lambda}(t)}^+.\label{ODE lambda part-2}
		\end{equation}
		%\end{subequations}
		We also find $A\bar{h}(0) = b$. Since $AL = 0$, it is not hard to see that we then have $A\bar{h}(t) = b$ for all $t \in [0,\infty)$. For the next part we write $G(\bar{h}) := G\big(\bar{h}(t)\big)$. %
		%\begin{equation*}
		%	G(\bar{h}) :=  F\big(\bar{h}(t)\big)  -  c\Big(\bar{h}(t)  -  \Pi_{\HH}\big(\bar{h}(t) \big) \Big) \! - \! \bar{b}(t)
		%\end{equation*}
		Analoguous to the proof of Proposition \ref{projected theorem}, convergence of $\bar{h}(t)$ can be analyzed by considering the Lyapunov function $V(\bar{h}) = \frac{1}{2} \norm{\bar{h} - h^*}$. Letting $X_{e \equiv 0}(\bar{h})$ denote the right-hand side of \eqref{eq:subspace-ODE} we obtain \jvmargin{need to address change in $G$ due to setting $b$ to zero.}
		\begin{align*}
			\nabla V &(\bar{h}) X_{e \equiv 0}(\bar{h}) = -(\bar{h} - h^*)^\top L G(\bar{h})	\\
			&= -(\bar{h} - h^*)^\top G(\bar{h}) + (\bar{h} - h^*)^\top (\sum_{i = 1}^{M}u_iu_i^\top ) G(\bar{h}).	
		\end{align*}
		Since $\{u_1,\cdots,u_{n}\}$ is an orthonormal basis for $\real^n$ it follows that for some $c_i \in \real$ we can write
		\begin{equation*}
			G(\bar{h}) = \sum_{i = 1}^M c_i u_i + \sum_{i = M+1}^n c_i u_i.
		\end{equation*}
		This gives us
		\begin{equation*}
			(\sum_{i = 1}^M u_iu_i^\top) G(\bar{h}) = \sum_{i = 1}^M c_i u_i.
		\end{equation*}
		Since each $u_i$ is in $\text{span}(a_1,\cdots,a_t)$ it follows that there exist $c_{i,j} \in \real$ such that $u_i = \sum_{j = 1}^l c_{i,j} a_j$. Therefore we have
		\begin{align*}
			(\bar{h} - h^*)^\top\sum_{i = 1}^M c_i u_i &= (\bar{h} - h^*)^\top\sum_{i = 1}^M \sum_{j = 1}^l c_i c_{i,j} a_j	\\
			&= \sum_{i = 1}^M \sum_{j = 1}^l c_i c_{i,j} (\bar{h} - h^*)^\top a_j	\\
			&= 0.
		\end{align*}
		The last equality here holds, since $A\bar{h} = A h^* = v$. Combining all of the above, we find
		\begin{align*}
			\nabla V (\bar{h}) X_{e \equiv 0}(\bar{h}) = -(\bar{h} - h^*)^\top G(\bar{h}).
		\end{align*}
		This, however, is exactly \eqref{vdot penalty}. The result therefore follows from  the arguments in the proof of Proposition \ref{penalty theorem}.
		%
		%However, the only difference between $\nabla V(\bar{x}) \dot{\bar{x}}$ when $\bar{x}$ follows the dynamics of \eqref{eq:ODE-h-lm} and when it follows the dynamics of \eqref{eq:ODE-h-lm-2} is that the term $(\bar{h} - h^*)^\top  \Big(H \big(\bar{h}(t), \bar{\lambda}(t), 0 \big)  - \bar{b}(t)  \Big)$ is replaced with $(\bar{h} - h^*)^\top L \Big( H \big(\bar{h}(t), \bar{\lambda}(t), 0 \big)  - \bar{b}(t) \Big)$. Since we have just shown these to be equal, the result follows from the proof of Proposition \ref{lagrange theorem}.
		%
		%\begin{align*}
		%	\frac{d}{d t} \bar{h}(t) &= F\big(\bar{h}(t)\big) \! - \! c\Big(\bar{h}(t)  \!- \! \Pi_{\HH}\big(\bar{h}(t) \big) \Big) \! - \! \bar{b}(t)	\\
		%	&+ \sum_{i \in [r]}u_iu_i^\top\Big(F\big(\bar{h}(t)\big) \! - \! c\Big(\bar{h}(t)  \!- \! \Pi_{\HH}\big(\bar{h}(t) \big) \Big) \! - \! \bar{b}(t)\Big).
		%
		%-L \Big( H\big(\bar{h}(t), &\bar{\lambda}(t), \bar{\mu}(t)\big)  - \bar{b}(t) \Big)	\\ 
		%&= H\big(\bar{h}(t), \bar{\lambda}(t), \bar{\mu}(t)\big)  - \bar{b}(t)	\\
		%&\enskip + \sum_{i \in [r]}u_iu_i^\top \Big( H\big(\bar{h}(t), \bar{\lambda}(t), \bar{\mu}(t)\big)  - \bar{b}(t) \Big). 
		%\end{align*}
		%Let $\{u_1,\cdots,u_r,w_{r+1},\cdots,w_{n}\}$ be an orthonormal basis for $\real^n$. It follows that for some $c_i \in \real$ we can write
		%\begin{equation*}
		%	H\big(\bar{h}(t), \bar{\lambda}(t), \bar{\mu}(t)\big)  - \bar{b}(t) = \sum_{i = 1}^r c_i u_i + \sum_{i = r+1}^n c_i w_i.
		%\end{equation*}
		%This gives us
		%\begin{equation*}
		%	\sum_{i \in [r]}u_iu_i^\top \Big( H\big(\bar{h}(t), \bar{\lambda}(t), \bar{\mu}(t)\big)  - \bar{b}(t) \Big) = \sum_{i \in [r]} c_i u_i.
		%\end{equation*}
		%Since each $u_i$ is in $\text{span}(a_1,\cdot,a_t)$ it follows that there exist $c_{i,j} \in \real$ such that $u_i = \sum_{j = 1}^t c_{i,j} a_j$. Therefore we have
		%\begin{align*}
		%	(\bar{h} - h^*)^\top\sum_{i \in [r]} c_i u_i &= (\bar{h} - h^*)^\top\sum_{i \in [r]} \sum_{j \in [t]} c_i c_{i,j} a_j	\\
		%	&= \sum_{i \in [r]} \sum_{j \in [t]} c_i c_{i,j} (\bar{h} - h^*)^\top	\\
		%	&= 0.
		%\end{align*}
		%The last equality here holds, since $A\bar{h} = A h^* = v$. Combining all of the above, we find
		%\begin{align*}
		%	(\bar{h} - h^*)^\top L \Big( &H \big(\bar{h}(t), \bar{\lambda}(t), 0 \big)  - \bar{b}(t) \Big)	\\ 
		%	&= (\bar{h} - h^*)^\top  \Big(H \big(\bar{h}(t), \bar{\lambda}(t), 0 \big)  - \bar{b}(t)  \Big).
		%\end{align*}
		%Analoguous to the proof of Proposition \ref{lagrange theorem}, convergence of $\bar{h}(t)$ can be analyzed by considering the Lyapunov function $V(\cdot)$ as given in \eqref{lyapunov function}. However, the only difference between $\nabla V(\bar{x}) \dot{\bar{x}}$ when $\bar{x}$ follows the dynamics of \eqref{eq:ODE-h-lm} and when it follows the dynamics of \eqref{eq:ODE-h-lm-2} is that the term $(\bar{h} - h^*)^\top  \Big(H \big(\bar{h}(t), \bar{\lambda}(t), 0 \big)  - \bar{b}(t)  \Big)$ is replaced with $(\bar{h} - h^*)^\top L \Big( H \big(\bar{h}(t), \bar{\lambda}(t), 0 \big)  - \bar{b}(t) \Big)$. Since we have just shown these to be equal, the result follows from the proof of Proposition \ref{lagrange theorem}.
	\end{proof}
	%	
	%Consider $\HH$ to be of the form
	%\begin{align*}
	%	\HH = \setdef{h \in \realnonnegative^n}{\ones_n^\top h = 1}.
	%\end{align*}
	%Let $\epsilon > 0$ be given and consider the map $\map{F^\epsilon}{\real^n}{\real}$ where each component is defined as
	%\begin{align*}
	%	F_i^\epsilon (h) = F_i(h) + \frac{1}{\epsilon} [-h_i]^+,
	%\end{align*}
	%for all $i \in \until{n}$. Consider the continuous-time system
	%\begin{align*}
	%	\dot h = - \Lap F^\epsilon(h).
	%\end{align*}
	%Questions:
	%\begin{itemize}
	%	\item What are the equilibrium points of the above dynamics? 
	%	\item Can we make epsilon small enough to push these equilibria close to the solution of the VI? Check Facchinei's book for similar penalty based approximation for solving VI. This looks like some perturbation analysis.
	%\end{itemize}
	

